Unsupervised 3D Pose Estimation with Geometric Self-Supervision

We present an unsupervised learning approach to recover 3D human pose from 2D skeletal joints extracted from a single image. Our method does not require any multi-view image data, 3D skeletons, correspondences between 2D-3D points, or use previously learned 3D priors during training. A lifting network accepts 2D landmarks as inputs and generates a corresponding 3D skeleton estimate. During training, the recovered 3D skeleton is reprojected on random camera viewpoints to generate new "synthetic" 2D poses. By lifting the synthetic 2D poses back to 3D and re-projecting them in the original camera view, we can define self-consistency loss both in 3D and in 2D. The training can thus be self supervised by exploiting the geometric self-consistency of the lift-reproject-lift process. We show that self-consistency alone is not sufficient to generate realistic skeletons, however adding a 2D pose discriminator enables the lifter to output valid 3D poses. Additionally, to learn from 2D poses "in the wild", we train an unsupervised 2D domain adapter network to allow for an expansion of 2D data. This improves results and demonstrates the usefulness of 2D pose data for unsupervised 3D lifting. Results on Human3.6M dataset for 3D human pose estimation demonstrate that our approach improves upon the previous unsupervised methods by 30% and outperforms many weakly supervised approaches that explicitly use 3D data.

==> discussions.tex <==


%\section{Discussion}
%\label{sect:discussions}
%\input{tableSupervised}

%It is well known that supervised approaches perform significantly better than unsupervised approaches on classification and regression tasks. For human 3D pose estimation, we do not expect our unsupervised method to outperform the state-of-the-art supervised approach~\cite{MartinezICCV2017}. However, our results are better than several previous published works that use 3D supervision as shown in Table~\ref{table:P2_sh_supervisedcomparison}. We have demonstrated the effectiveness of a relatively simple adversarial training framework using only 2D pose landmarks to achieve this.

%While the focus of this work is on unsupervised learning from 2D poses alone, we are very encouraged \st{to see} \rmvk{by the fact} that our results are competitive with the best in class supervised approaches. In fact, our approach comes to within 1.1mm of the error reported by~\cite{MartinezICCV2017} on the ground truth 2D detections as shown in Table~\ref{table:supervised}. We also experimented with a na\"ive ensemble algorithm that took snapshots of our model with errors ranging between 38.2mm to 40.6mm and averaged the 3D poses for each input. This simple algorithm reduced the error to 36.3mm, surpassing the state-of-the-art results of 37.1mm (Table~\ref{table:supervised}). %As a reference, in the Human3.6M dataset on

%This appears to be close to the lower limit of MJPJE error on the Human3.6~\.

%In summary, we believe that we have significantly pushed the state of art in 3D pose estimation using unsupervised learning. This paves way for new research directions that can extend this work by combining supervised, weakly-supervised, and unsupervised frameworks (\ie, semi-supervised) for lifting 2D poses to 3D skeletons.

%While the focus of this work is on unsupervised learning from 2D poses alone, we conducted a small proof-of-concept experiment to augment the learning with limited amount of supervised data. We fine-tuned our un-supervised model with $40K$ 2D-3D correspondences using L2 regression loss as in~\cite{MartinezICCV2017}. Table~\ref{table:supervised} shows the average MJPJE error on Protocal-2 with previous supervised approaches using ground-truth 2D points. This further reduced the error to $36.5$mm, surpassing the performance of~\cite{MartinezICCV2017}. Thus, we believe that there is significant potential in further combining our un-supervised approach with existing weakly-supervised and fully-supervised approaches.

%In future, we would like to extend our approach to semi-supervised approaches by combining better 3D priors and 3D information.

\begin{table}[t]
	\centering
	\begin{tabularx}{\textwidth}{ l *{8}{Y} }
		
		\toprule
		Method & Direct. & Discuss & Eat & Greet & Phone & Photo & Pose & Purchase \\
		\midrule
		Akhter \& Black~\cite{akhter2015pose} & 199.2 & 177.6 & 161.8 & 197.8 & 176.2 & 186.5 & 195.4 & 167.3 \\
		Ramakrishna~\etal~\cite{ramakrishna2012reconstructing} & 137.4 & 149.3 & 141.6 & 154.3 & 157.7 & 158.9 & 141.8 & 158.1 \\
		Zhou~\etal~\cite{Zhou_2016_CVPR} & 99.7 & 95.8 & 87.9 & 116.8 & 108.3 & 107.3 & 93.5 & 95.3\\
		% Moreno-Noguer~\cite{distance-matrix} (SA) 14j & 69.5 & 80.2 & 78.2 & 87.0 & 100.8 & 102.7 & 76.0 & 69.7 & 104.7 & 113.9 & 89.7 & 98.5 & 79.2 & 82.4 & 77.2 & 87.3\\
		% Newer CVPR version
		% Moreno-Noguer~\cite{distance-matrix} (SA) 14j & 67.5 & 79.0 & 76.5 & 83.1 & 97.4 & 74.6 & 72.0 & 102.4 & 116.7 & 87.7 & 100.4 & 94.6 & 75.2 & 82.7 & 74.9 & 85.6\\
		Bogo~\etal~\cite{keep-it-simpl} & 62.0 & 60.2 & 67.8 & 76.5 & 92.1 & 77.0 & 73.0 & 75.3 \\
		Moreno-Noguer~\cite{Moreno-Noguer_2017_CVPR} & 66.1 & 61.7 & 84.5 & 73.7 & 65.2 & 67.2 & 60.9 & 67.3\\
		Martinez~\etal~\cite{MartinezICCV2017} & {44.8} & {52.0} & {44.4} & {50.5} &	{61.7} & {59.4} & {45.1} & {41.9} \\
		\midrule
		\ouremph{Ours (\textit{Unsupervised})} & \ouremph{60.2}&	\ouremph{60.7}&	\ouremph{59.2}&	\ouremph{65.1}&	\ouremph{65.5}&	\ouremph{63.8}&	\ouremph{59.4}&	\ouremph{59.4} \\
		\bottomrule
		
		\toprule	
		Method & Sit & SitD & Smoke & Wait & Walk & WalkD & WalkP & Avg.\\
		\midrule
		Akhter \& Black~\cite{akhter2015pose}& 160.7 & 173.7 & 177.8 & 181.9 & 176.2 & 198.6 & 192.7 & 181.1\\
		Ramakrishna~\etal~\cite{ramakrishna2012reconstructing} & 168.6 & 175.6 & 160.4 & 161.7 & 150.0 & 174.8 & 150.2 & 157.3\\
		Zhou~\etal~\cite{Zhou_2016_CVPR}&  109.1 & 137.5 & 106.0 & 102.2 & 106.5 & 110.4 & 115.2 & 106.7\\
		Bogo~\etal~\cite{keep-it-simpl}  &  100.3 & 137.3 & 83.4 & 77.3 & 86.8 & 79.7 & 87.7 & 82.3\\
		Moreno-Noguer~\cite{Moreno-Noguer_2017_CVPR} & 103.5 & 74.6 & 92.6 & 69.6 & 71.5 & 78.0 & 73.2 & 74.0\\
		Martinez~\etal~\cite{MartinezICCV2017} & {66.3} & {77.6} & {54.0} & {58.8} & {49.0} & {35.9} & {40.7} &  {52.1}\\
		\midrule
		\ouremph{Ours (\textit{Unsupervised})} &	\ouremph{69.1}&	\ouremph{88.0}&	\ouremph{64.8}&	\ouremph{60.8}&	\ouremph{64.9}&	\ouremph{63.9}&	\ouremph{65.2}&	\ouremph{64.6}\\
		\bottomrule
		%\end{tabular}
	\end{tabularx}
	\vspace{1mm}
	\caption{Comparison of our approach to other supervised methods on Human3.6M under \textbf{Protocol 2} using detected 2D keypoints. The results of all approaches are obtained from~\cite{MartinezICCV2017}. Our \textit{unsupervised} approach outperforms most supervised methods that use 3D data and comes close to the state of the art supervised approach of~\cite{MartinezICCV2017}.}
	\label{table:P2_sh_supervisedcomparison}
	%\vspace{-5mm}
\end{table}


\begin{table}[b]%[htb!]
	\small
		\centering
	%\begin{tabular}{cccc}
	\begin{tabularx}{0.97\textwidth}{ *{4}{Y} }
		\toprule
		Moreno-Noguer	& Martinez~\etal	& \multicolumn{2}{c}{Ours (Unsupervised)} \\
		\cite{Moreno-Noguer_2017_CVPR} & \cite{MartinezICCV2017} &  { (Single Model)} & { (Ensemble)} \\
		\midrule
		62.2	& \underline{37.1} & 38.2 & {\bf 36.3} \\
		\bottomrule
	%\end{tabular}
\end{tabularx}
\vspace{1mm}
\caption{Comparison of our unsupervised results to the state of the art fully supervised approaches under Protocol 2 using ground truth 2D inputs. Our unsupervised model has error within 1.1mm of the best supervised approach, and outperforms the same with a na\"ive ensemble approach.}
\label{table:fully-supervised}
\label{table:supervised}
%\vspace{-6mm}
\end{table}
	




%%% this is single col
%%\begin{sidewaystable}
%\begin{table*}
%	\centering
%	\footnotesize
%	\hspace{-3mm}
%	\tabcolsep=0.6mm
%	%\tiny
%	\begin{tabular}{@{}lrrrrrrrrrrrrrrrr@{}}
%		\toprule
%		Protocol \#2 & Direct. & Discuss & Eating & Greet & Phone & Photo & Pose & Purch. & Sitting & SitingD & Smoke & Wait & WalkD & Walk & WalkT & Avg\\
%		\midrule
%		Akhter \& Black~\cite{akhter2015pose}* (MA) 14j & 199.2 & 177.6 & 161.8 & 197.8 & 176.2 & 186.5 & 195.4 & 167.3 & 160.7 & 173.7 & 177.8 & 181.9 & 176.2 & 198.6 & 192.7 & 181.1\\
%		Ramakrishna~\etal~\cite{ramakrishna2012reconstructing}* (MA) 14j & 137.4 & 149.3 & 141.6 & 154.3 & 157.7 & 158.9 & 141.8 & 158.1 & 168.6 & 175.6 & 160.4 & 161.7 & 150.0 & 174.8 & 150.2 & 157.3\\
%		Zhou~\etal~\cite{zhou2016sparseness}* (MA) 14j & 99.7 & 95.8 & 87.9 & 116.8 & 108.3 & 107.3 & 93.5 & 95.3 & 109.1 & 137.5 & 106.0 & 102.2 & 106.5 & 110.4 & 115.2 & 106.7\\
%		% Moreno-Noguer~\cite{distance-matrix} (SA) 14j & 69.5 & 80.2 & 78.2 & 87.0 & 100.8 & 102.7 & 76.0 & 69.7 & 104.7 & 113.9 & 89.7 & 98.5 & 79.2 & 82.4 & 77.2 & 87.3\\
%		% Newer CVPR version
%		% Moreno-Noguer~\cite{distance-matrix} (SA) 14j & 67.5 & 79.0 & 76.5 & 83.1 & 97.4 & 74.6 & 72.0 & 102.4 & 116.7 & 87.7 & 100.4 & 94.6 & 75.2 & 82.7 & 74.9 & 85.6\\
%		Bogo~\etal~\cite{keep-it-simpl} (MA) 14j & 62.0 & 60.2 & 67.8 & 76.5 & 92.1 & 77.0 & 73.0 & 75.3 & 100.3 & 137.3 & 83.4 & 77.3 & 86.8 & 79.7 & 87.7 & 82.3\\
%		Moreno-Noguer~\cite{Moreno-Noguer_2017_CVPR} (MA) 14j & 66.1 & 61.7 & 84.5 & 73.7 & 65.2 & 67.2 & 60.9 & 67.3 & 103.5 & 74.6 & 92.6 & 69.6 & 71.5 & 78.0 & 73.2 & 74.0\\
%		%Pavlakos~\etal~\cite{volumetric} (MA) 17j & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & \underline{51.9}\\
%		Martinez~\etal~\cite{MartinezICCV2017} (SH detections) (SA) 14j & \textbf{44.8} & \textbf{52.0} & \textbf{44.4} & \textbf{50.5} &	\textbf{61.7} & \textbf{59.4} & \textbf{45.1} & \textbf{41.9} &	\textbf{66.3} & \textbf{77.6} & \textbf{54.0} & \textbf{58.8} & \textbf{49.0} & \textbf{35.9} & \textbf{40.7} &  \textbf{52.1}\\
%%		\midrule
%%		Ours (SH detections) (SA) 17j & 50.1 &  59.5 & 51.3 & 56.9 & 68.5 & 67.5 & 51.0 & 47.2 & 68.5 & 85.6 & 61.2 & 67.0 & 55.1 & 41.1 & 45.5 & 58.5  \\
%%		% Ours (SH detections) (MA) 17j & \bf{45.9} & \bf{50.1} & \underline{52.2} & \bf{53.5} & \bf{64.2} & \bf{65.1} & \bf{46.2} & \bf{46.7} & \bf{68.3} & \bf{81.0} & \bf{58.0} & \bf{51.6} & \underline{56.5} & \underline{45.0} & \underline{51.0} & \underline{55.7}\\
%%		Ours (SH detections) (MA) 17j & \underline{42.2}&	\underline{48.0}&	\underline{49.8}&	\underline{50.8}&	\underline{61.7}&	\underline{60.7}&	\underline{44.2}&	\underline{43.6}&	\underline{64.3}&	\underline{76.5}&	\underline{55.8}&	\underline{49.1}&	\underline{53.6}&	\underline{40.8}&	\underline{46.4}&	52.5\\
%%		Ours (SH detections FT) (MA) 17j & \bf{39.5} & \bf{43.2}&	\bf{46.4}&	\bf{47.0}&	\bf{51.0}&	\bf{56.0}&	\bf{41.4}&	\bf{40.6}&	\bf{56.5}&	\bf{69.4}&	\bf{49.2}&	\bf{45.0}&	\bf{49.5}&	\bf{38.0}&	\bf{43.1}&	\bf{47.7}\\
%%		\midrule
%		Ours (SH detections) (SA) 14j & \underline{60.2}&	\underline{60.7}&	\underline{59.2}&	\underline{65.1}&	\underline{65.5}&	\underline{63.8}&	\underline{59.4}&	\underline{59.4}&	\underline{69.1}&	\underline{88.0}&	\underline{64.8}&	\underline{60.8}&	\underline{64.9}&	\underline{63.9}&	\underline{65.2}&	\underline{64.6}\\
%		\bottomrule
%	\end{tabular}
%	
%	\vspace{3mm}
%	\caption{Detailed results on Human3.6M~\cite{h36m} under protocol \#2 (rigid alignment in post-processing).
%		The 14j (17j) annotation indicates that the body model considers 14 (17) body joints.
%		%The \texttt{xx}j annotation indicates that the body model considers \texttt{xx} body joints.
%		The results of all approaches are obtained from the original
%		papers, except for (*), which were obtained from~\cite{keep-it-simpl}.}
%	\label{tab:h36m_2}
%\end{table*}
%%\end{sidewaystable}
%%\begin{table*}[t]

